Recommendations for Visualization Recommendations: Exploring Preferences and Priorities in Public Health

The promise of visualization recommendation systems is that analysts will be automatically provided with relevant and high-quality visualizations that will reduce the work of manual exploration or chart creation. However, little research to date has focused on what analysts value in the design of visualization recommendations. We interviewed 18 analysts in the public health sector and explored how they made sense of a popular in-domain dataset. in service of generating visualizations to recommend to others. We also explored how they interacted with a corpus of both automatically- and manually-generated visualization recommendations, with the goal of uncovering how the design values of these analysts are reflected in current visualization recommendation systems. We find that analysts champion simple charts with clear takeaways that are nonetheless connected with existing semantic information or domain hypotheses. We conclude by recommending that visualization recommendation designers explore ways of integrating context and expectation into their systems.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> content/table.tex <==
\begin{table}[htbp]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ |c|c|c|c|c|c|c|c|c|c| }
\hline
ID & mark & X & Y & color & (encoding type 4, attribute) & (encoding type 5, attribute)\\
\hline\hline 
\multirow{3}{4em}{P1} & bar & Diastolic\_Blood\_pressure(mm\_Hg) [mean] & Gender & Gender & (row, Caffeine(mg)) &  \\ 
& boxplot & Alcohol(gm) & Feeling\_Down\_or\_Depressed & Feeling\_Down\_or\_Depressed & & \\ 
& bar & Annual\_Family\_Income [binned] & Annual\_Family\_Income(dollar) [binned, count] & & &  \\ 
\hline\hline 
\multirow{3}{4em}{P2} & arc & & & Age [binned] & (theta, Experience\_Hearing\_Problem [count]) &  \\ 
& line & Annual\_Family\_Income(dollar) & Body\_Mass\_Index(kg/m**2) [mean] & & & \\ 
& point & Body\_Mass\_Index(kg/m**2) & (Total\_Fat(gm), Total\_Sugars(gm), Water\_Per\_Day(gm)) & & &  \\ 
\hline\hline 
\multirow{3}{4em}{P3} & bar & Education\_Level & (Total\_Sugars(gm) [mean], Energy(kcal) [mean]) & & &  \\ 
& bar & Have\_Diabetes & (Total\_Sugars(gm) [mean], Energy(kcal) [mean]) & Have\_Diabetes & & \\ 
& line & Annual\_Family\_Income(dollar) & (Total\_Sugars(gm) [mean], Energy(kcal) [mean]) & & &  \\ 
\hline\hline 
\multirow{3}{4em}{P4} & bar & Could\_Not\_Afford\_Food & Body\_Mass\_Index(kg/m**2) [mean] & & &  \\  
& boxplot & Annual\_Family\_Income(dollar) & Body\_Mass\_Index(kg/m**2) & & & \\
& - & - & - & - & - &  \\\hline\hline
\multirow{3}{4em}{P5} & bar & Experience\_Sleeping\_Issue [count, stacked] & Experience\_Sleeping\_Issue & Could\_Not\_Afford\_Food & &  \\ 
& circle & Gender [count] &  & Gender & (row, Education\_Level) & \\ 
& line & Annual\_Family\_Income(dollar) & Total\_Sugars(gm) [mean] & & &  \\ 
\hline\hline 
\multirow{3}{4em}{P6} & line & Age & Body\_Mass\_Index(kg/m**2) [mean] & Gender & &  \\ 
& boxplot & Have\_Or\_Had\_Heart\_Attack & Diastolic\_Blood\_pressure(mm\_Hg) & & (column, Gender) & \\ 
& line & Age & Caffeine(mg) [mean] & Gender & &  \\ 
\hline\hline 
\multirow{3}{4em}{P8} & bar & Experience\_Tooth\_Aching & Total\_Sugars(gm) [mean] & & &  \\ 
& bar & Have\_Diabetes & Alcohol(gm) [mean] & & & \\ 
& point & Body\_Mass\_Index(kg/m**2) & Alcohol(gm) & & &  \\ 
\hline\hline 
\multirow{3}{4em}{P9} & arc & &  & Could\_Not\_Afford\_Food & (theta, Could\_Not\_Afford\_Food [count]) &  (facet, Age [binned])\\ 
& bar & Annual\_Family\_Income(dollar) & Feeling\_Down\_or\_Depressed [count] & Feeling\_Down\_or\_Depressed & & (facet, Gender) \\ 
& bar & Gender & Could\_Not\_Afford\_Food [count] & Could\_Not\_Afford\_Food & &  \\ 
\hline\hline 
\multirow{3}{4em}{P11} & line & Age & Diastolic\_Blood\_pressure(mm_Hg) [mean] & Could\_Not\_Afford\_Food &  &  \\ 
& line & Age & Diastolic\_Blood\_pressure(mm\_Hg) [mean] & Gender & &  \\ 
& line & Age & Diastolic\_Blood\_pressure(mm\_Hg) [mean] & Annual\_Family\_Income(dollar) [binned] & &  \\
\hline\hline 
\multirow{3}{4em}{P12} & bar & Body\_Mass\_Index(kg/m**2) & Have\_Or\_Had\_Heart\_Attack [count] & Have\_Or\_Had\_Heart\_Attack &  &  \\ 
& bar & Education\_Level & Have\_Or\_Had\_Heart\_Attack [count] & Have\_Or\_Had\_Heart\_Attack & &  \\ 
& bar & Have\_Diabetes [count] & Annual\_Family\_Income(dollar) [binned] & Have\_Diabetes & &  \\
\hline\hline 
\multirow{3}{4em}{P13} & bar & Have\_Diabetes [count] & Age [binned] &  &  (facet, Have\_Diabetes) &  \\ 
& bar & Have\_Diabetes [count] & Gender &  &  (facet, Have\_Diabetes) &  \\ 
& bar & Have\_Diabetes [count] & Could\_Not\_Afford\_Food &  &  (facet, Have\_Diabetes) &  \\ 
\hline\hline 
\multirow{3}{4em}{P14} & bar & Age [binned] & Have\_Diabetes [count] &  & &  \\ 
& bar & Body\_Mass\_Index [binned] & Have\_Or\_Had\_Heart\_Attack [count] &  &  &  \\ 
& line & Annual\_Family\_Income(dollar) & Have\_Diabetes [count] &  &  &  \\ 
\hline\hline 
\multirow{3}{4em}{P15} & line & Annual\_Family\_Income(dollar) & Body\_Mass\_Index [mean] &  & &  \\ 
& bar & Have\_Diabetes & Annual\_Family\_Income(dollar) [mean] & Have\_Diabetes &  &  \\ 
& bar & Experience\_Sleeping\_Issue & Feeling\_Down\_or\_Depressed [count] &  &  &  \\ 
\hline\hline 
\multirow{3}{4em}{P16} & arc & & & Annual\_Family\_Income(dollar) & (theta, Annual\_Family\_Income(dollar) [count, stacked]) & (facet, Have\_Or\_Had\_Heart\_Attack)  \\ 
& line & Diastolic\_Blood\_pressure(mm\_Hg) & Body\_Mass\_Index [mean] & Gender &  &  \\ 
& bar & Annual\_Family\_Income(dollar) & Total\_Sugars(gm) [mean] &  &  &  \\ 
\hline\hline 
\multirow{3}{4em}{P18} & bar & Annual\_Family\_Income(dollar) [binned] & Experience\_Tooth\_Aching [count, stacked] & Experience\_Tooth\_Aching & &  \\ 
& arc &  &  & Feeling\_Down\_or\_Depressed & (theta, Feeling\_Down\_or\_Depressed [count]) & (facet, Gender) \\ 
& bar & Could\_Not\_Afford\_Food & Could\_Not\_Afford\_Food [count] & Could\_Not\_Afford\_Food & (facet, Age [binned]) &  \\
\hline\hline
\multirow{3}{4em}{P19} & bar & Education\_Level & Body\_Mass\_Index(kg/m**2) [mean] & Education\_Level & &  \\ 
& arc &  &  & Feeling\_Down\_or\_Depressed & (theta, Feeling\_Down\_or\_Depressed [count]) & (facet, Gender) \\ 
& bar & Have\_Diabetes & Annual\_Family\_Income(dollar) [mean] & Have\_Diabetes & &  \\ 
\hline\hline 
\end{tabular}
}
\caption{Participant sketches translated into Vega-lite specifications. The enclosed function(s) in square brackets $[]$, following an attribute, were applied to it. \leilani{Do we really need to add a whole table here? Would it not suffice to include the specifications on OSF and mention they are in the repository?}}
\label{tab:full-participant-sketches-list}
\end{table}


\begin{table}[htbp]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ |c|c|c|c|c|c|c|c|c|c|c|c| }
\hline
Overall Rank & Visualization ID & Source & Chart Type & X & Y & Color & (encoding type 4, attribute)\\
\hline\hline
1 & G & Voyager & Bar & Body\_Mass\_Index(kg/m**2) [binned] & Water\_Per\_Day(gm) [mean] & Water\_Per\_Day(gm) [mean] & \\\hline 
2 & C & Human & Line & Age & Energy(kcal) [mean], Body\_Mass\_Index(kg/m**2) [mean] & & \\\hline
3 & H & Human & Heatmap & Body\_Mass\_Index(kg/m**2) & Energy(kcal) & & \\\hline 
4 & A & Dziban & Scatterplot & Total\_Fat(gm) & Diastolic\_Blood\_pressure(mm\_Hg) & & \\\hline 
5 & B & Human & Boxplot & Age [binned] & Annual\_Family\_Income(dollar) [mean] & Education\_Level &  \\\hline 
6 & I & Human & Heatmap & Experience\_Hearing\_Problem & Annual\_Family\_Income & Age [mean] & \\\hline 
7 & F & Dziban & Heatmap & Body\_Mass\_Index [binned] & Diastolic\_Blood\_pressure(mm\_Hg) & & size, * \\\hline 
8 & E & Voyager & Heatmap  & Diastolic\_Blood\_pressure(mm\_Hg) [binned] & Total\_Sugars(gm) & Age & \\\hline 
9 & J & Human & Table  & Gender [count], Age [mean], Energy(kcal) [mean], Body\_Mass\_Index(kg/m**2) [mean] & &  & \\\hline 
10 & D & Dziban & Scatterplot  & Water\_Per\_Day(gm) & & Water\_Per\_Day(gm) &  \\\hline 
\end{tabular}}\caption{\label{tab:overall-rank}Gallery of Recommendations, ranked by our interviewees. Overall rank is determined by summing all interview ranking data grouped by Visualization ID then sorting in descending order.}
\end{table}
